Strategies in PRholog

PRholog is an experimental extension of logic programming with strategic conditional transformation rules, combining Prolog with Rholog calculus. The rules perform nondeterministic transformations on hedges. Queries may have several results that can be explored on backtracking. Strategies provide a control on rule applications in a declarative way. With strategy combinators, the user can construct more complex strategies from simpler ones. Matching with four different kinds of variables provides a flexible mechanism of selecting (sub)terms during execution. We give an overview on programming with strategies in PRholog and demonstrate how rewriting strategies can be expressed.

==> eptcsdata.tex <==
\providecommand{\event}{M. Fernandez (Ed.): 9th Int. Workshop on Reduction Strategies\\
in Rewriting and Programming (WRS'09)}
\providecommand{\volume}{15}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{32}
\providecommand{\eid}{3}

